Global Solutions to the Ultra-Relativistic Euler Equations

We prove a global existence theorem for the $3\times 3$ system of relativistic Euler equations in one spacial dimension. It is shown that in the ultra-relativistic limit, there is a family of equations of state that satisfy the second law of thermodynamics for which solutions exist globally. With this limit and equation of state, which includes equations of state for both an ideal gas and one dominated by radiation, the relativistic Euler equations can be analyzed by a Nishida-type method leading to a large data existence theorem, including the entropy and particle number evolution, using a Glimm scheme. Our analysis uses the fact that the equations of state are of the form $p=p(n,S)$, but whose form simplifies to $p=a^{2}\rho$ when viewed as a function of $\rho$ alone.

==> EntropyInteraction.tex <==
Proof Here

